The Disk Orientations of Perseus Protostellar Multiples at 8 au Resolution

We present a statistical characterization of circumstellar disk orientations toward 12 protostellar multiple systems in the Perseus molecular cloud using the Atacama Large Millimeter/submillimeter Array at Band 6 (1.3 mm) with a resolution of 25 mas (8 au). This exquisite resolution enabled us to resolve the compact inner disk structures surrounding the components of each multiple system and to determine the projected 3-D orientation of the disks (position angle and inclination) to high precision. We performed a statistical analysis on the relative alignment of disk pairs to determine whether the disks are preferentially aligned or randomly distributed. We considered three subsamples of the observations selected by the companion separations, a <100 au, a >500 au, and a < 10,000 au. We found for the compact (< 100 au) subsample, the distribution of orientation angles is best described by an underlying distribution of preferentially aligned sources (within 30deg) but does not rule out distributions with 40% misaligned sources. The wide companion (>500 au) subsample appears to be consistent with a distribution of 40%-80% preferentially aligned sources. Similarly, the full sample of systems with companions (a< 10, 000 au) is most consistent with a fractional ratio of at most 80% preferentially aligned source and rules out purely randomly aligned distributions. Thus our results imply the compact sources (<100 au) and the wide companions (>500 au) are statistically different.

==> cover.tex <==
\author[0000-0002-9239-6422]{Nickalas K. Reynolds}
\affiliation{Homer L. Dodge Department of Physics and Astronomy, The University of Oklahoma, 440 W Brooks St, Norman, OK, 73019 USA}

\author[0000-0002-6195-0152]{John J. Tobin}
\author[0000-0002-9209-8708]{Patrick D. Sheehan}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Rd, Charlottesville, VA 22903 USA}

\author[0000-0001-7474-6874]{Sarah I. Sadavoy}
\affiliation{Department of Physics, Engineering Physics and Astronomy, Queen’s University, Kingston, ON, K7L 3N6, Canada}

\author[0000-0002-4540-6587]{Leslie W. Looney}
\affiliation{Department of Astronomy, University of Illinois, 1002 W. Green St., Urbana, IL 61801, USA }

\author[0000-0001-7474-6874]{Kaitlin M. Kratter}
\affiliation{Department of Astronomy, /Steward Observatory, University of Arizona 933 North Cherry Avenue, Rm. N204, Tucson, AZ 85721-0065}

\author{Zhi-Yun Li}
\affiliation{Department of Astronomy, University of Virginia, 530 McCormick Rd., Charlottesville, VA 22903, USA}

\author[0000-0003-3172-6763]{Dominique M. Segura-Cox}\thanks{NSF Astronomy and Astrophysics Postdoctoral Fellow}
\affiliation{Department of Astronomy, University of Texas, 2515 Speedway Stop Austin, TX 78712}
\affiliation{Max Planck Institute for extraterrestrial Physics,Giessenbachstrasse 1, D-85748 Garching, Bayern, Germany}

\author[0000-0001-5272-5888]{Nathan A. Kaib}
\affiliation{Homer L. Dodge Department of Physics and Astronomy, The University of Oklahoma, 440 W Brooks St, Norman, OK, 73019 USA}


\begin{acknowledgments}

NKR, JJT, and NAK gratefully acknowledge support from NSF AST-1814762. LWL acknowledges support from NSF AST-2108794. ZYL is supported in part by NASA 80NSSC20K0533 and NSF AST-2307199. DMSC is supported by an NSF Astronomy and Astrophysics Postdoctoral Fellowship under award AST-2102405. DMSC is grateful for support from the Max Planck Society. This paper makes use of the following ALMA data: ADS/JAO.ALMA\#2019.1.01425.S and 2017.1.00337.S. ALMA is a partnership of ESO (representing its member states), NSF (USA) and NINS (Japan), together with NRC (Canada), MOST and ASIAA (Taiwan), and KASI (Republic of Korea), in cooperation with the Republic of Chile. The Joint ALMA Observatory is operated by ESO, AUI/NRAO and NAOJ. The National Radio Astronomy Observatory is a facility of the National Science Foundation operated under cooperative agreement by Associated Universities, Inc.

\end{acknowledgments}

==> zimgtex_3mmcontzoom.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{zimg_combined_continuum_zoom_3mm.pdf}
    \caption{ALMA cycle 5 3~mm continuum images of the Perseus multiples, with Per-emb-2, Per-emb-5, and Per-emb-18 reconstructed with superuniform weighting, with the zoom-in image-size specified. A 0\farcs1~(30~au)~scalebar is shown in the lower left and the respective restoring beam (average size$\approx$ 0\farcs09$\times$0\farcs04)\space is shown in the lower right.}\label{fig:3mmcont}
\end{figure}

==> zimgtex_contjvec.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{zimg_combined_continuum_jvector.pdf}
    \caption{Summary of the various source fitting techniques overlaid on the same image as Figure~\ref{fig:cont}. The orientation vectors (angles orthogonal to the disk major axis) are indicated as colored lines for each of the fit sources. The cyan line indicates the image-plane derived orientation vectors while the dashed red line indicates the \textit{uv}-visibility derived orientation vectors.}\label{fig:jveccontinuum}
\end{figure}

==> zimgtex_rac1999vla20.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.475\textwidth]{zimg_RAC1999VLA20-continuum-multiplot.pdf}
    \caption{The source RAC1999 VLA20 which is found within the field of SVS13 A. However it is believed to be an extra-galactic source \citep[][]{1999rodriguezanglada,2016tobinlooney}\space so, for the purpose of the analysis conducted in the paper. A 0\farcs1~(30~au)~scalebar is shown in the lower left and the representative beam is in the lower right. The white contours denote the 3~$\sigma$~level, where the 1~$\sigma=0.90$~$\mu$Jy~\beam. The colormap is square-root scaled.}\label{fig:rac1999}
\end{figure}

==> ztable_13mmtimeonsource.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{deluxetable}{lccc}
\tablecaption{1.3~mm Time on Sources}
\tablehead{
\colhead{Name} & \colhead{\# Scans} & \colhead{Time} & \colhead{Identifier}\\
\colhead{} & \colhead{} & \colhead{(minutes)} & \colhead{}
}
\startdata
L1448IRS1 & 12 & 9.07 & (2)\\
Per-emb-2 & 21 & 13.46 & (1)\\
Per-emb-5 & 20 & 13.51 & (1)\\
NGC1333IRAS2A & 21 & 14.36 & (1)\\
Per-emb-17 & 13 & 9.02 & (2)\\
Per-emb-18 & 22 & 14.31 & (1)\\
Per-emb-22 & 12 & 9.07 & (2)\\
L1448IRS3B & 11 & 9.12 & (2)\\
L1448IRS3C & 14 & 8.97 & (2)\\
Per-emb-35 & 20 & 14.41 & (1)\\
NGC1333IRAS2B & 18 & 14.52 & (1)\\
SVS13A & 20 & 14.41 & (1)\\
\enddata
\tablecomments{Identifier (1) corresponds to the Member Observation Unit Set (MOUS) of uid://A001/X1465/Xd60 and (2) corresponds to uid://A001/X1465/Xd63.}\label{table:13mmtimeonsource}
% GENERATED BY COMPILE_EB_TABLES.PY
% 1677212214.5345783
\end{deluxetable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> ztable_fullresult-100_10000_500-allsources-m4-imtable.tex <==

% AD KS Statistics
%    fullresult-100_10000_500-allsources-m4
%    Number of resamples: 10000
%    Types of fitting: dict_keys(['imfit', 'uv-visibility fitting'])
%    Number of real sources: {'imfit': ['L1448IRS3C--source-1---L1448IRS3C--source-2', 'L1448IRS3B--source-1---L1448IRS3B--source-2', 'L1448IRS3B--source-3---L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3A--source-1---L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3C--source-1___L1448IRS3C--source-2---L1448IRS3A--source-1___L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'SVS13A--source-1---SVS13A--source-2', 'SVS13A--source-3---SVS13A--source-1___SVS13A--source-2', 'SVS13B--source-1---SVS13A--source-3___SVS13A--source-1___SVS13A--source-2', 'NGC1333IRAS2B--source-1---NGC1333IRAS2B--source-2', 'NGC1333IRAS2A--source-1---NGC1333IRAS2A--source-2', 'NGC1333IRAS2B--source-1___NGC1333IRAS2B--source-2---NGC1333IRAS2A--source-1___NGC1333IRAS2A--source-2', 'Per-emb-18--source-1---Per-emb-18--source-2', 'Per-emb-21--source-1---Per-emb-18--source-1___Per-emb-18--source-2', 'Per-emb-35--source-1---Per-emb-35--source-2', 'Per-emb-2--source-4---Per-emb-2--source-5'], 'uv-visibility fitting': ['L1448IRS3C--source-1---L1448IRS3C--source-2', 'L1448IRS3B--source-1---L1448IRS3B--source-2', 'L1448IRS3B--source-3---L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3A--source-1---L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3C--source-1___L1448IRS3C--source-2---L1448IRS3A--source-1___L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'SVS13A--source-1---SVS13A--source-2', 'SVS13A--source-3---SVS13A--source-1___SVS13A--source-2', 'SVS13B--source-1---SVS13A--source-3___SVS13A--source-1___SVS13A--source-2', 'NGC1333IRAS2B--source-1---NGC1333IRAS2B--source-2', 'NGC1333IRAS2A--source-1---NGC1333IRAS2A--source-2', 'NGC1333IRAS2B--source-1___NGC1333IRAS2B--source-2---NGC1333IRAS2A--source-1___NGC1333IRAS2A--source-2', 'Per-emb-18--source-1---Per-emb-18--source-2', 'Per-emb-21--source-1---Per-emb-18--source-1___Per-emb-18--source-2', 'Per-emb-35--source-1---Per-emb-35--source-2', 'Per-emb-2--source-4---Per-emb-2--source-5']}
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{deluxetable}{lrrr|rrr|rrr}
\tablecaption{Model image-plane Fitting Statistics}
\tablehead{
\colhead{Fractional Alignment} & \multicolumn{3}{c}{$<$100 au} & \multicolumn{3}{c}{$<$10,000 au} & \multicolumn{3}{c}{$>$500 au}\\
\colhead{} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$}
}
\startdata
C$_{1.00}$ UC$_{0.00}$ & 77.7 & 52.3 & 40.9 & 3.2 & 0.0 & 64.0 & 50.7 & 0.8 & 84.7\\
C$_{0.90}$ UC$_{0.10}$ & 94.1 & 97.2 & 19.4 & 32.1 & 15.8 & 61.6 & 91.9 & 82.6 & 84.4\\
C$_{0.80}$ UC$_{0.20}$ & 99.5 & 100.0 & 7.9 & 83.5 & 83.0 & 47.6 & 99.8 & 100.0 & 39.0\\
C$_{0.70}$ UC$_{0.30}$ & 100.0 & 100.0 & 5.4 & 99.6 & 99.9 & 46.1 & 100.0 & 100.0 & 28.2\\
C$_{0.60}$ UC$_{0.40}$ & 100.0 & 100.0 & 4.7 & 100.0 & 100.0 & 47.8 & 100.0 & 100.0 & 25.9\\
C$_{0.50}$ UC$_{0.50}$ & 99.7 & 99.9 & 4.0 & 99.8 & 100.0 & 45.1 & 99.9 & 100.0 & 23.3\\
C$_{0.40}$ UC$_{0.60}$ & 95.4 & 99.0 & 3.7 & 97.8 & 99.4 & 42.2 & 97.8 & 99.5 & 21.3\\
C$_{0.30}$ UC$_{0.70}$ & 84.9 & 92.3 & 3.6 & 87.9 & 88.6 & 38.3 & 84.6 & 83.6 & 19.4\\
C$_{0.20}$ UC$_{0.80}$ & 75.2 & 80.4 & 3.2 & 71.3 & 64.6 & 32.2 & 63.4 & 49.9 & 16.0\\
C$_{0.10}$ UC$_{0.90}$ & 63.4 & 65.0 & 3.0 & 56.0 & 40.6 & 27.2 & 45.0 & 23.6 & 13.7\\
C$_{0.00}$ UC$_{1.00}$ & 58.8 & 58.5 & 2.9 & 51.8 & 33.1 & 26.2 & 41.2 & 18.8 & 13.1\\
\enddata
\tablecomments{Same as Table~\ref{table:stats10010000500im}, except using the image-plane results from the deconvolved \textit{imfit}\space task from CASA.}\label{table:stats10010000500im}
% GENERATED FROM MAKE_HISTOGRAM_DOTPROD.PY
% 1688447451.3783867
\end{deluxetable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Groupings
%########imfit
%L1448IRS3C--source-1,L1448IRS3A--source-1,L1448IRS3B--source-1,L1448IRS3B--source-2,L1448IRS3B--source-3,L1448IRS3C--source-1,L1448IRS3C--source-2
%SVS13A--source-1,SVS13A--source-1,SVS13A--source-2,SVS13A--source-3,SVS13B--source-1
%NGC1333IRAS2B--source-1,NGC1333IRAS2A--source-1,NGC1333IRAS2A--source-2,NGC1333IRAS2B--source-1,NGC1333IRAS2B--source-2
%Per-emb-18--source-1,Per-emb-18--source-1,Per-emb-18--source-2,Per-emb-21--source-1
%Per-emb-35--source-1,Per-emb-35--source-1,Per-emb-35--source-2
%Per-emb-2--source-4,Per-emb-2--source-4,Per-emb-2--source-5
%########uv-visibility fitting
%L1448IRS3C--source-1,L1448IRS3A--source-1,L1448IRS3B--source-1,L1448IRS3B--source-2,L1448IRS3B--source-3,L1448IRS3C--source-1,L1448IRS3C--source-2
%SVS13A--source-1,SVS13A--source-1,SVS13A--source-2,SVS13A--source-3,SVS13B--source-1
%NGC1333IRAS2B--source-1,NGC1333IRAS2A--source-1,NGC1333IRAS2A--source-2,NGC1333IRAS2B--source-1,NGC1333IRAS2B--source-2
%Per-emb-18--source-1,Per-emb-18--source-1,Per-emb-18--source-2,Per-emb-21--source-1
%Per-emb-35--source-1,Per-emb-35--source-1,Per-emb-35--source-2
%Per-emb-2--source-4,Per-emb-2--source-4,Per-emb-2--source-5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%LINKS
%########imfit
%L1448IRS3A--source-1:L1448IRS3B--source-2: 2,151 au
%L1448IRS3B--source-1:L1448IRS3A--source-1..L1448IRS3B--source-2: 1,140 au
%L1448IRS3B--source-3:L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 600 au
%L1448IRS3C--source-1:L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 6,146 au
%L1448IRS3C--source-2:L1448IRS3C--source-1..L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 3,132 au
%SVS13A--source-2:SVS13A--source-3: 1,522 au
%SVS13A--source-1:SVS13A--source-2..SVS13A--source-3: 843 au
%SVS13B--source-1:SVS13A--source-1..SVS13A--source-2..SVS13A--source-3: 4,128 au
%NGC1333IRAS2A--source-2:NGC1333IRAS2B--source-2: 9,243 au
%NGC1333IRAS2B--source-1:NGC1333IRAS2A--source-2..NGC1333IRAS2B--source-2: 4,699 au
%NGC1333IRAS2A--source-1:NGC1333IRAS2B--source-1..NGC1333IRAS2A--source-2..NGC1333IRAS2B--source-2: 7,075 au
%Per-emb-18--source-2:Per-emb-21--source-1: 3,966 au
%Per-emb-18--source-1:Per-emb-18--source-2..Per-emb-21--source-1: 2,004 au
%Per-emb-35--source-1:Per-emb-35--source-2: 570 au
%Per-emb-2--source-4:Per-emb-2--source-5: 575 au
%########uv-visibility fitting
%L1448IRS3A--source-1:L1448IRS3B--source-2: 2,149 au
%L1448IRS3B--source-1:L1448IRS3A--source-1..L1448IRS3B--source-2: 1,139 au
%L1448IRS3B--source-3:L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 596 au
%L1448IRS3C--source-1:L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 6,148 au
%L1448IRS3C--source-2:L1448IRS3C--source-1..L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 3,133 au
%SVS13A--source-2:SVS13A--source-3: 1,522 au
%SVS13A--source-1:SVS13A--source-2..SVS13A--source-3: 842 au
%SVS13B--source-1:SVS13A--source-1..SVS13A--source-2..SVS13A--source-3: 4,127 au
%NGC1333IRAS2B--source-2:NGC1333IRAS2A--source-2: 9,243 au
%NGC1333IRAS2B--source-1:NGC1333IRAS2B--source-2..NGC1333IRAS2A--source-2: 4,699 au
%NGC1333IRAS2A--source-1:NGC1333IRAS2B--source-1..NGC1333IRAS2B--source-2..NGC1333IRAS2A--source-2: 7,075 au
%Per-emb-18--source-2:Per-emb-21--source-1: 3,966 au
%Per-emb-18--source-1:Per-emb-18--source-2..Per-emb-21--source-1: 2,001 au
%Per-emb-35--source-1:Per-emb-35--source-2: 570 au
%Per-emb-2--source-4:Per-emb-2--source-5: 578 au
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> ztable_fullresult-100_10000_500-allsources-m4-uvtable.tex <==

% AD KS Statistics
%    fullresult-100_10000_500-allsources-m4
%    Number of resamples: 10000
%    Types of fitting: dict_keys(['imfit', 'uv-visibility fitting'])
%    Number of real sources: {'imfit': ['L1448IRS3C--source-1---L1448IRS3C--source-2', 'L1448IRS3B--source-1---L1448IRS3B--source-2', 'L1448IRS3B--source-3---L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3A--source-1---L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3C--source-1___L1448IRS3C--source-2---L1448IRS3A--source-1___L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'SVS13A--source-1---SVS13A--source-2', 'SVS13A--source-3---SVS13A--source-1___SVS13A--source-2', 'SVS13B--source-1---SVS13A--source-3___SVS13A--source-1___SVS13A--source-2', 'NGC1333IRAS2B--source-1---NGC1333IRAS2B--source-2', 'NGC1333IRAS2A--source-1---NGC1333IRAS2A--source-2', 'NGC1333IRAS2B--source-1___NGC1333IRAS2B--source-2---NGC1333IRAS2A--source-1___NGC1333IRAS2A--source-2', 'Per-emb-18--source-1---Per-emb-18--source-2', 'Per-emb-21--source-1---Per-emb-18--source-1___Per-emb-18--source-2', 'Per-emb-35--source-1---Per-emb-35--source-2', 'Per-emb-2--source-4---Per-emb-2--source-5'], 'uv-visibility fitting': ['L1448IRS3C--source-1---L1448IRS3C--source-2', 'L1448IRS3B--source-1---L1448IRS3B--source-2', 'L1448IRS3B--source-3---L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3A--source-1---L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'L1448IRS3C--source-1___L1448IRS3C--source-2---L1448IRS3A--source-1___L1448IRS3B--source-3___L1448IRS3B--source-1___L1448IRS3B--source-2', 'SVS13A--source-1---SVS13A--source-2', 'SVS13A--source-3---SVS13A--source-1___SVS13A--source-2', 'SVS13B--source-1---SVS13A--source-3___SVS13A--source-1___SVS13A--source-2', 'NGC1333IRAS2B--source-1---NGC1333IRAS2B--source-2', 'NGC1333IRAS2A--source-1---NGC1333IRAS2A--source-2', 'NGC1333IRAS2B--source-1___NGC1333IRAS2B--source-2---NGC1333IRAS2A--source-1___NGC1333IRAS2A--source-2', 'Per-emb-18--source-1---Per-emb-18--source-2', 'Per-emb-21--source-1---Per-emb-18--source-1___Per-emb-18--source-2', 'Per-emb-35--source-1---Per-emb-35--source-2', 'Per-emb-2--source-4---Per-emb-2--source-5']}
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{deluxetable}{lrrr|rrr|rrr}
\tablecaption{Model uv-visibility Fitting Statistics}
\tablehead{
\colhead{Fractional Alignment} & \multicolumn{3}{c}{$<$100 au} & \multicolumn{3}{c}{$<$10,000 au} & \multicolumn{3}{c}{$>$500 au}\\
\colhead{} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$} & \colhead{\%$_{KS}$} & \colhead{\%$_{AD}$} & \colhead{\%$_{ES}$}
}
\startdata
C$_{1.00}$ UC$_{0.00}$ & 100.0 & 100.0 & 32.1 & 12.8 & 0.0 & 87.6 & 95.5 & 5.1 & 98.3\\
C$_{0.90}$ UC$_{0.10}$ & 100.0 & 100.0 & 4.4 & 85.5 & 72.7 & 99.7 & 100.0 & 100.0 & 99.4\\
C$_{0.80}$ UC$_{0.20}$ & 100.0 & 100.0 & 0.1 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 90.1\\
C$_{0.70}$ UC$_{0.30}$ & 100.0 & 100.0 & 0.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 25.5\\
C$_{0.60}$ UC$_{0.40}$ & 99.8 & 99.6 & 0.0 & 100.0 & 100.0 & 99.8 & 100.0 & 100.0 & 13.5\\
C$_{0.50}$ UC$_{0.50}$ & 97.6 & 94.7 & 0.0 & 100.0 & 100.0 & 99.2 & 100.0 & 100.0 & 8.2\\
C$_{0.40}$ UC$_{0.60}$ & 56.7 & 69.9 & 0.0 & 95.3 & 99.6 & 94.0 & 96.8 & 99.0 & 6.3\\
C$_{0.30}$ UC$_{0.70}$ & 40.6 & 15.0 & 0.0 & 57.8 & 56.4 & 64.9 & 73.7 & 46.4 & 5.1\\
C$_{0.20}$ UC$_{0.80}$ & 16.0 & 1.4 & 0.0 & 22.3 & 8.0 & 38.0 & 41.2 & 3.2 & 3.8\\
C$_{0.10}$ UC$_{0.90}$ & 3.5 & 0.1 & 0.0 & 8.2 & 0.6 & 21.5 & 17.8 & 0.1 & 2.7\\
C$_{0.00}$ UC$_{1.00}$ & 2.8 & 0.0 & 0.0 & 5.6 & 0.2 & 17.2 & 14.4 & 0.0 & 2.4\\
\enddata
\tablecomments{The fractional alignment column details the fractional ratio of aligned vs randomly aligned as indicated by the subscripts. \%$_{KS}$, \%$_{AD}$, and \%$_{ES}$ correspond to the \% of resampled observation dot products that cannot reject the null hypothesis in favour of the alternative for Kolmogorov-Smirnov, Anderson-Darling, and Epps-Singleton statistical tests respectively. The rejection criteria is evaluated at 0.3\%. The total number of resampled observation dot products are 10,000. The null hypothesis tested is the empirical distributions and the corresponding constructed fractional distributions are drawn from the same underlying distribution.}\label{table:stats10010000500uv}
% GENERATED FROM MAKE_HISTOGRAM_DOTPROD.PY
% 1688447451.3499436
\end{deluxetable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Groupings
%########imfit
%L1448IRS3C--source-1,L1448IRS3A--source-1,L1448IRS3B--source-1,L1448IRS3B--source-2,L1448IRS3B--source-3,L1448IRS3C--source-1,L1448IRS3C--source-2
%SVS13A--source-1,SVS13A--source-1,SVS13A--source-2,SVS13A--source-3,SVS13B--source-1
%NGC1333IRAS2B--source-1,NGC1333IRAS2A--source-1,NGC1333IRAS2A--source-2,NGC1333IRAS2B--source-1,NGC1333IRAS2B--source-2
%Per-emb-18--source-1,Per-emb-18--source-1,Per-emb-18--source-2,Per-emb-21--source-1
%Per-emb-35--source-1,Per-emb-35--source-1,Per-emb-35--source-2
%Per-emb-2--source-4,Per-emb-2--source-4,Per-emb-2--source-5
%########uv-visibility fitting
%L1448IRS3C--source-1,L1448IRS3A--source-1,L1448IRS3B--source-1,L1448IRS3B--source-2,L1448IRS3B--source-3,L1448IRS3C--source-1,L1448IRS3C--source-2
%SVS13A--source-1,SVS13A--source-1,SVS13A--source-2,SVS13A--source-3,SVS13B--source-1
%NGC1333IRAS2B--source-1,NGC1333IRAS2A--source-1,NGC1333IRAS2A--source-2,NGC1333IRAS2B--source-1,NGC1333IRAS2B--source-2
%Per-emb-18--source-1,Per-emb-18--source-1,Per-emb-18--source-2,Per-emb-21--source-1
%Per-emb-35--source-1,Per-emb-35--source-1,Per-emb-35--source-2
%Per-emb-2--source-4,Per-emb-2--source-4,Per-emb-2--source-5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%LINKS
%########imfit
%L1448IRS3A--source-1:L1448IRS3B--source-2: 2,151 au
%L1448IRS3B--source-1:L1448IRS3A--source-1..L1448IRS3B--source-2: 1,140 au
%L1448IRS3B--source-3:L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 600 au
%L1448IRS3C--source-1:L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 6,146 au
%L1448IRS3C--source-2:L1448IRS3C--source-1..L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 3,132 au
%SVS13A--source-2:SVS13A--source-3: 1,522 au
%SVS13A--source-1:SVS13A--source-2..SVS13A--source-3: 843 au
%SVS13B--source-1:SVS13A--source-1..SVS13A--source-2..SVS13A--source-3: 4,128 au
%NGC1333IRAS2A--source-2:NGC1333IRAS2B--source-2: 9,243 au
%NGC1333IRAS2B--source-1:NGC1333IRAS2A--source-2..NGC1333IRAS2B--source-2: 4,699 au
%NGC1333IRAS2A--source-1:NGC1333IRAS2B--source-1..NGC1333IRAS2A--source-2..NGC1333IRAS2B--source-2: 7,075 au
%Per-emb-18--source-2:Per-emb-21--source-1: 3,966 au
%Per-emb-18--source-1:Per-emb-18--source-2..Per-emb-21--source-1: 2,004 au
%Per-emb-35--source-1:Per-emb-35--source-2: 570 au
%Per-emb-2--source-4:Per-emb-2--source-5: 575 au
%########uv-visibility fitting
%L1448IRS3A--source-1:L1448IRS3B--source-2: 2,149 au
%L1448IRS3B--source-1:L1448IRS3A--source-1..L1448IRS3B--source-2: 1,139 au
%L1448IRS3B--source-3:L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 596 au
%L1448IRS3C--source-1:L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 6,148 au
%L1448IRS3C--source-2:L1448IRS3C--source-1..L1448IRS3B--source-3..L1448IRS3B--source-1..L1448IRS3A--source-1..L1448IRS3B--source-2: 3,133 au
%SVS13A--source-2:SVS13A--source-3: 1,522 au
%SVS13A--source-1:SVS13A--source-2..SVS13A--source-3: 842 au
%SVS13B--source-1:SVS13A--source-1..SVS13A--source-2..SVS13A--source-3: 4,127 au
%NGC1333IRAS2B--source-2:NGC1333IRAS2A--source-2: 9,243 au
%NGC1333IRAS2B--source-1:NGC1333IRAS2B--source-2..NGC1333IRAS2A--source-2: 4,699 au
%NGC1333IRAS2A--source-1:NGC1333IRAS2B--source-1..NGC1333IRAS2B--source-2..NGC1333IRAS2A--source-2: 7,075 au
%Per-emb-18--source-2:Per-emb-21--source-1: 3,966 au
%Per-emb-18--source-1:Per-emb-18--source-2..Per-emb-21--source-1: 2,001 au
%Per-emb-35--source-1:Per-emb-35--source-2: 570 au
%Per-emb-2--source-4:Per-emb-2--source-5: 578 au
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

